Faster Meta Update Strategy for Noise-Robust Deep Learning

It has been shown that deep neural networks are prone to overfitting on biased training data. Towards addressing this issue, meta-learning employs a meta model for correcting the training bias. Despite the promising performances, super slow training is currently the bottleneck in the meta learning approaches. In this paper, we introduce a novel Faster Meta Update Strategy (FaMUS) to replace the most expensive step in the meta gradient computation with a faster layer-wise approximation. We empirically find that FaMUS yields not only a reasonably accurate but also a low-variance approximation of the meta gradient. We conduct extensive experiments to verify the proposed method on two tasks. We show our method is able to save two-thirds of the training time while still maintaining the comparable or achieving even better generalization performance. In particular, our method achieves the state-of-the-art performance on both synthetic and realistic noisy labels, and obtains promising performance on long-tailed recognition on standard benchmarks.

==> tables/more_results_on_cifar10_cifar100.tex <==
\begin{table}[t]
	\centering
	\small
	\begin{tabular}{|l|cc|cc|}
	\hline
	\multirow{2}{*}{Method} & \multicolumn{2}{|c|}{CIFAR-10} & \multicolumn{2}{|c|}{CIFAR-100} \\
	\cline{2-5}
	                   & 40\% & 60\% & 40\% & 60\% \\
	\hline
	\hline
	\small{DivideMix}  & 95.06 & 94.46 & 75.15 & 71.41  \\
	                   & $\pm$0.14 & $\pm$0.21 & $\pm$0.12 & $\pm$0.61 \\
	\hline
	\small{MW-Net + Pseudo-clean} & 93.64 & 92.91 & 74.61 & 70.55 \\
	                     & $\pm$0.35 & $\pm$0.15 & $\pm$0.25 & $\pm$0.57\\
	\hline\hline
	\textbf{Ours}        & 95.37 & 94.97 & 75.91 & 73.58 \\
	                     & $\pm$0.15 & $\pm$0.11 & $\pm$0.19 & $\pm$0.28 \\
	\hline
	\end{tabular}
	\caption{Results on CIFAR-10 and CIFAR-100. ``Pseudo-clean'' refers to the pseudo-clean label set constructed by GMMs. Percentage numbers denote the noise rate.}\label{tab:comp_baselines}
\end{table}


==> tables/sota_clothing1m.tex <==
\begin{table}[t]
	\centering
	\small
	\begin{tabular}{|l|c|}
		\hline
		Method & Accuracy (\%)\\
		\hline
		F-correction~\cite{patrini2017making} & 69.84 \\
        \hline
        JoCoR~\cite{wei2020combating} & 70.30 \\
        \hline
        M-correction~\cite{arazo2019unsupervised} & 71.00  \\ 
        \hline
        MLC~\cite{wang2020training} & 71.06\\
        \hline
        Joint-Optim~\cite{tanaka2018joint} & 72.16  \\
        \hline
        MLNT~\cite{li2019learning} & 73.47 \\
        \hline
        P-correction~\cite{yi2019probabilistic} & 73.49 \\
        \hline
		MW-Net~\cite{shu2019meta} & 73.72 \\
        \hline
        MentorMix~\cite{jiang2020beyond} & 74.30 \\
		\hline\hline
		\textbf{Ours} & \textbf{74.43} \\
		\hline
	\end{tabular}
	\caption{Top-1 Accuracy on Clothing1M.}\label{tab:clothing1m}
\end{table}

